Keyframes First, Motion Second: Revisiting Compressed-Domain Video Captioning under Limited Supervision

Compressed-domain video captioners such as CoCap read the H.264 bitstream directly: a pretrained encoder reads the keyframes (I-frames), while motion and residual encoders, trained from scratch, turn the codec's motion vectors and residuals into action tokens. This motion branch costs decoding time and supervision, both scarce on edge devices. We ask when it pays off under limited supervision. In a controlled study on 2,500 VATEX training clips, we fix a frozen SigLIP 2 keyframe encoder, a GPT-2 caption decoder and the training schedule, vary only the visual tokens the decoder receives (34 configurations), and report held-out test CIDEr with paired bootstrap intervals and three seeds. Motion encoders trained from scratch bring no measurable benefit: CoCap-style action tokens change CIDEr by -0.55 (95% CI [-2.3, +1.2]), and six other uses of motion do not help. Warm-started from a model trained on 48x the caption samples, they add +1.3 CIDEr on average, though not significantly across seeds, and only while the keyframe tokens stay frozen. Reading the keyframes better matters more: fine-tuning SigLIP 2's own attention-pooling head adds 5.4 CIDEr, and one to eight such tokens beat the 16 CoCap-style tokens on every seed while decoding only I-frames (7.3 ms instead of 44-114 ms per clip). The same holds on MSVD's full split in CoCap's own video encoding, where the readout leads by 14.2 CIDEr and action tokens bring no reliable gain, also with clean single-reference motion vectors. Under limited supervision, keyframes come first and motion second.

==> figures/all_configs.tex <==
%
\multicolumn{9}{@{}l}{\textit{CoCap-style and context tokens}} \\
Context tokens only, no action & 8 & 37.87 & 29.21 & 21.77 & 19.59 & 43.87 & 12.8 & 0.90 \\
CoCap-style (8 context + 8 action) & 16 & 37.30 & 28.66 & 21.88 & 19.76 & 44.20 & 13.6 & -- \\
\midrule
\multicolumn{9}{@{}l}{\textit{Average pooling and token merging}} \\
ToMe, one-shot & 392 & 47.30 & 36.75 & \textbf{25.96} & 20.70 & \textbf{45.93} & 9.2 & 0.37 \\
ToMe, gradual & 392 & 45.23 & 35.23 & 24.69 & 20.53 & 45.47 & 6.4 & 0.38 \\
ToMe, parameter-free attention & 16 & 42.83 & 31.02 & 23.62 & 19.86 & 44.84 & 7.2 & 0.39 \\
ToMe & 16 & 42.50 & 30.39 & 23.42 & 19.67 & 44.88 & 5.0 & 0.40 \\
ToMe, medoid merge & 16 & 40.79 & 28.78 & 22.86 & 19.38 & 44.35 & 5.2 & 0.31 \\
Average pooling & 392 & 30.60 & 22.25 & 20.34 & 18.29 & 42.57 & 31.2 & 0.57 \\
\midrule
\multicolumn{9}{@{}l}{\textit{Attention-pooling (MAP) readouts}} \\
ToMe-cluster readout, fine-tuned & 16 & 46.76 & \textbf{37.25} & 24.18 & \textbf{20.80} & 45.25 & 15.2 & 0.44 \\
16-query readout, fine-tuned & 16 & \textbf{48.62} & 36.14 & 23.62 & 20.62 & 45.17 & 16.2 & 0.90 \\
16-query readout, spread start & 16 & 46.19 & 36.04 & 23.53 & 20.65 & 45.04 & 12.4 & 1.00 \\
8-query readout, fine-tuned & 8 & 44.80 & 35.75 & 23.27 & 20.59 & 44.82 & 10.0 & 1.00 \\
Per-I-frame readout, fine-tuned & 8 & 44.93 & 35.44 & 23.83 & 20.59 & 45.14 & 13.0 & 0.81 \\
ToMe-cluster readout, frozen & 392 & 45.46 & 34.93 & 24.03 & 20.44 & 44.97 & 12.4 & 0.53 \\
32-query readout, fine-tuned & 32 & 44.34 & 34.69 & 23.29 & 20.42 & 44.97 & 11.0 & 1.00 \\
One-query readout, fine-tuned & 1 & 45.28 & 34.13 & 23.29 & 20.26 & 44.88 & 11.0 & -- \\
ToMe-cluster readout, random start & 16 & 43.67 & 32.77 & 23.13 & 19.99 & 44.89 & 11.6 & 0.30 \\
ToMe, mean then trained head & 16 & 42.60 & 31.10 & 22.29 & 19.76 & 44.01 & 16.2 & 0.45 \\
16-query readout, random start & 16 & 41.63 & 30.73 & 22.38 & 19.71 & 44.21 & 11.0 & 1.00 \\
ToMe-cluster readout, frozen & 16 & 41.93 & 30.48 & 21.90 & 19.70 & 44.25 & 12.8 & 0.55 \\
One-query readout, random start & 1 & 39.12 & 29.97 & 22.23 & 19.69 & 44.26 & 12.0 & -- \\
Per-I-frame readout, random start & 8 & 38.76 & 29.95 & 22.39 & 19.61 & 44.28 & 12.0 & 0.80 \\
\midrule
\multicolumn{9}{@{}l}{\textit{Fewer keyframes}} \\
One-query readout, 4 I-frames & 1 & 44.50 & 33.64 & 24.34 & 20.32 & 45.07 & 3.2 & -- \\
One-query readout, 2 I-frames & 1 & 41.30 & 29.49 & 21.35 & 19.50 & 43.62 & 6.2 & -- \\
One-query readout, 1 I-frame & 1 & 38.89 & 28.66 & 21.88 & 19.11 & 43.43 & 5.8 & -- \\
ToMe over 4 I-frames & 16 & 39.51 & 28.36 & 22.26 & 19.43 & 43.86 & 7.4 & 0.40 \\
\midrule
\multicolumn{9}{@{}l}{\textit{Uses of codec motion (encoders trained from scratch)}} \\
Residual-guided ToMe & 392 & 43.58 & 33.47 & 24.52 & 20.29 & 45.68 & 5.0 & 0.37 \\
Motion-guided ToMe & 392 & 43.80 & 33.40 & 24.51 & 20.29 & 45.36 & 5.2 & 0.38 \\
ToMe + weighted motion statistics & 16 & 40.53 & 30.10 & 23.11 & 19.75 & 44.25 & 8.0 & 0.40 \\
ToMe + motion statistics & 16 & 41.44 & 28.78 & 22.85 & 19.56 & 44.11 & 6.8 & 0.40 \\
8 ToMe + 8 action tokens & 16 & 37.99 & 28.40 & 20.94 & 19.69 & 43.62 & 10.4 & 0.38 \\
Motion-guided ToMe & 16 & 37.61 & 27.46 & 23.03 & 19.30 & 44.12 & 4.4 & 0.15 \\
ToMe + weighted motion statistics & 392 & 35.22 & 25.58 & 20.87 & 18.83 & 43.43 & 42.2 & 0.37 \\
Action-guided ToMe & 392 & 32.93 & 25.23 & 21.95 & 18.73 & 43.83 & 34.2 & 0.35 \\

